End-to-end Neural Coreference Resolution

We introduce the first end-to-end coreference resolution model and show that it significantly outperforms all previous work without using a syntactic parser or hand-engineered mention detector. The key idea is to directly consider all spans in a document as potential mentions and learn distributions over possible antecedents for each. The model computes span embeddings that combine context-dependent boundary representations with a head-finding attention mechanism. It is trained to maximize the marginal likelihood of gold antecedent spans from coreference clusters and is factored to enable aggressive pruning of potential mentions. Experiments demonstrate state-of-the-art performance, with a gain of 1.5 F1 on the OntoNotes benchmark and by 3.1 F1 using a 5-model ensemble, despite the fact that this is the first approach to be successfully trained with no external resources.

==> figures/task.tex <==
\begin{figure}[t!]
\centering
\begin{examplebox}
\textcolor{black!50}{
\cospan{(\att{1}{The} \att{5}{``}\att{25}{USS} \att{60}{Cole}\att{11}{''})} has (arrived) back at ((the (Mississippi) shipyard) where \cospan{(\att{100}{she})} was built). ((ABC's) John M. Wethy) reports (tonight) before ((the attack) on \cospan{(\att{1}{the} \att{100}{ship})}, (the crew) (failed) to (take) at least 25\% of ((the 80 different steps) to protect \cospan{(\att{1}{the} \att{100}{ship})}) before (landing) in (Yemen).\vspace{6pt}
\textcolor{black}{\hrule height 0.8pt}
\vspace{6pt}
After (George W. Bush) is (sworn) in, (Bill Clinton) will head to (New York). (The President) has (said) \cospan{((\att{0}{he}) \att{53}{and} (((\att{0}{his}) \att{1}{wife})\att{2}{,} \att{28}{now} (\att{0}{a} (\att{0}{New} \att{1}{York}) \att{5}{senator})))} will (spend) (weekends) at ((\cospan{(\att{100}{their})} house) in (Chappaqua)). (Mr. Clinton) will also spend time at (his) presidential library in (Arkansas). (He) says (he) will (come) to (Washington), ``every now and then.''}
\end{examplebox}
\caption{Visualized model predictions from the development set. Brackets indicate spans with high mention scores. Bolded spans indicate mentions that belong to one of the predicted clusters. The redness of each word indicates the weights of mention heads learned by the model. The top example shows head preferences that correspond well with traditional definitions. The bottom example shows head preferences there are more task specific, where coordination is an important signal for coreference.
\mike{This is interesting, but I'm not sure it's the most exciting thing to put on the first page. How about an example where rule-based mention detectors screw up?}
}
\label{fig:task}
\end{figure}
